CascadeXML: Rethinking Transformers for End-to-end Multi-resolution Training in Extreme Multi-label Classification

Extreme Multi-label Text Classification (XMC) involves learning a classifier that can assign an input with a subset of most relevant labels from millions of label choices. Recent approaches, such as XR-Transformer and LightXML, leverage a transformer instance to achieve state-of-the-art performance. However, in this process, these approaches need to make various trade-offs between performance and computational requirements. A major shortcoming, as compared to the Bi-LSTM based AttentionXML, is that they fail to keep separate feature representations for each resolution in a label tree. We thus propose CascadeXML, an end-to-end multi-resolution learning pipeline, which can harness the multi-layered architecture of a transformer model for attending to different label resolutions with separate feature representations. CascadeXML significantly outperforms all existing approaches with non-trivial gains obtained on benchmark datasets consisting of up to three million labels. Code for CascadeXML will be made publicly available at \url{https://github.com/xmc-aalto/cascadexml}.

==> Algorithm.tex <==
\begin{algorithm}
\SetKwInput{KwData}{Input}
\SetKwInput{KwResult}{Return}
\DontPrintSemicolon
\SetNoFillComment
\caption{Algorithm for \textsc{CascadeXML}}\label{alg:Cascade}
\KwData{X, Y}
$\hat{\mathbf{Z}}_l = \mathbf{v}_l/\left\lVert \mathbf{v}_l \right\rVert \textrm{; where} \; \mathbf{v}_l = \sum_{i:y_{i,l}=1}\Phi_{tfidf}(\mathbf{x}_i), \; \forall l \in [L]$\;
$\{\mathbf{C}^t\}_{t=1}^{T} \gets \textrm{2-means-clustering}(\hat{\mathbf{Z})}$\;
$\textrm{Generate} \{\mathbf{Y}^t\}_{t=1}^{T}$\;
\While{$\textrm{not convergence}$}{
    $\boldsymbol{\theta}^{[1..T]} \gets \Phi(\mathbf{X})$\;
    $\textrm{loss} \gets 0$\;
    \For{$t \; \textrm{in} \; 1,2,...,T$}{
        \eIf{$t = 1$}{
            % $\mathbf{S}^1 \gets [1, 2, .... K^1]$\;
            $\mathbf{P}^1 \gets (\mathbf{W}^1)^\top \boldsymbol{\theta}^1$ \quad \tcc{Dense predictions}
            $\mathbf{Y}_s^1 \gets \mathbf{Y}^1$\ \ \quad\quad \tcc{All labels for dense predictions}
        }{
            % \tcc{Shortlist clusters for projection to next resolution}
            $\mathbf{C}^{(t-1,t)}_{s} \gets \textrm{shortlist}(\mathbf{C}^{(t-1,t)}, \mathbf{S}^{t-1})$\ \quad\quad \tcc{Shortlist clusters}
            
            $\mathbf{S}_\textrm{W}^t \gets \mathbf{S}_L^{t-1} \mathbf{C}^{(t-1,t)}_{s}$\ \quad\quad \tcc{Create candidate OVA classifier shortlist}
            
            $\mathbf{W}^t_s = \textrm{shortlist}(\mathbf{W}^t,\ \mathbf{S}_\textrm{W}^t)$ \quad \ \quad \tcc{Shortlist candidate OVA classifiers}
            
            $\mathbf{P}^t = (\mathbf{W}^t_s)^\top\ \boldsymbol{\theta}^t$ \quad \quad\quad\quad\quad\quad \tcc{Sparse predictions} 
            
            $\mathbf{Y}_s^t \gets \textrm{shortlist}(\mathbf{Y}^t,\ \mathbf{S}^t)$ \quad\quad \tcc{Shortlist labels for sparse evaluation}
        }
        $\mathbf{S}_L^t \gets \textrm{binarize} (\textrm{Top}(\mathbf{P}^t, \ k^t)) + \mathbf{Y}_s^t)$ \quad \tcc{Add $\mathbf{Y}_s^t$ only during training}
        
        $\textrm{loss} \gets \textrm{loss} + \alpha^t\mathcal{L}(\mathbf{P}^t, \mathbf{Y}_s^t)$\;
        % $\mathbf{P}^t \gets \textrm{Top}(\mathbf{P}^t, \; k^t)$\;
    }
    $\Phi, \{\mathbf{W}\}^T_{t=1} \gets \textrm{argmin}_{\Phi, \{\mathbf{W}\}^T_{t=1}}\textrm{loss}$\;
}
\KwResult{$\Phi, \{\mathbf{W}\}^T_{t=1}, \{\mathbf{C}\}^T_{t=1}$}
\end{algorithm}


% \begin{algorithm}
% \SetKwInput{KwData}{Input}
% \SetKwInput{KwResult}{Return}
% \DontPrintSemicolon
% \SetNoFillComment
% \caption{Shortlisting Function}\label{alg:cap}
% \KwData{M: Matrix, S: Shortlist}
% $\mathbf{M}_s \gets \textrm{Empty List} $

% \For{$i \in \mathbf{S}$}{
%     \If{$\mathbf{S}_{i} \neq 0$}{
%         $\mathbf{M}_s \gets \mathbf{M}_i$\;
%     }
% }
% \KwResult{$\mathbf{M}_s$ : Matrix with only shortlisted rows}
% \end{algorithm}



% \begin{algorithm}
% \SetKwInput{KwData}{Input}
% \SetKwInput{KwResult}{Return}
% \DontPrintSemicolon
% \SetNoFillComment
% \caption{Algorithm for \textsc{CascadeXML}}\label{alg:cap}
% \KwData{X, Y}
% $\hat{\mathbf{Z}}_l = \mathbf{v}_l/\left\lVert \mathbf{v}_l \right\rVert \textrm{; where} \; \mathbf{v}_l = \sum_{i:y_{i,l}=1}\Phi_{tfidf}(\mathbf{x}_i), \; \forall l \in [L]$\;
% $\{\mathbf{C}^t\}_{t=1}^{T} \gets \textrm{2-means-clustering}(\hat{\mathbf{Z})}$\;
% $\textrm{Generate} \{\mathbf{Y}^t\}_{t=1}^{T}$\;
% \While{$\textrm{not convergence}$}{
%     $\boldsymbol{\theta}^{[1..T]} \gets \Phi(\mathbf{X})$\;
%     $\textrm{loss} \gets 0$\;
%     \For{$t \; \textrm{in} \; 1,2,...T$}{
%         \eIf{$t = 1$}{
%             $\mathbf{S}^1 \gets [1, 2, .... K^1]$\;
%             $\mathbf{P}^1 \gets (\mathbf{W}^1)^\top \boldsymbol{\theta}^1$ \quad \tcc{Dense predictions}
%             $\mathbf{Y}_s^1 \gets \mathbf{Y}^1$\ \ \quad\quad \tcc{All labels for dense predictions}
%         }{
%             \tcc{Shortlist clusters for projection to next resolution}
%             $\mathbf{C}^{(t-1,t)}_{s} \gets \textrm{shortlist}(\mathbf{C}^{(t-1,t)}, \mathbf{S}^{t-1})$\;
%             $\mathbf{\hat{P}}^t \gets \mathbf{P}^{t-1}\mathbf{C}^{(t-1,t)}_{s} + \mathbf{Y}^t$\ \quad\quad \tcc{Add $\mathbf{Y}^t$ only during training}
%             $\mathbf{S}^t \gets \textrm{binarize} (\textrm{Top}(\mathbf{\hat{P}}^t, \ k^t))$ \quad \tcc{Create shortlist for forward pass}
%             $\mathbf{W}^t_s = \textrm{shortlist}(\mathbf{W}^t,\ \mathbf{S}^t)$ \quad \ \quad \tcc{Shortlist candidate OVA classifiers}
%             $\mathbf{P}^t = (\mathbf{W}^t_s)^\top\ \boldsymbol{\theta}^t$ \quad \quad\quad\quad\quad \tcc{Sparse predictions}
%             $\mathbf{Y}_s^t \gets \textrm{shortlist}(\mathbf{Y}^t,\ \mathbf{S}^t)$ \quad\quad \tcc{Shortlisted labels for sparse predictions}
%         }
%         $\textrm{loss} \gets \textrm{loss} + \alpha^t\mathcal{L}(\mathbf{P}^t, \mathbf{Y}_s^t)$\;
%         % $\mathbf{P}^t \gets \textrm{Top}(\mathbf{P}^t, \; k^t)$\;
%     }
%     $\Phi, \{\mathbf{W}\}^T_{t=1} \gets \textrm{argmin}_{\Phi, \{\mathbf{W}\}^T_{t=1}}\textrm{loss}$\;
% }
% \KwResult{$\Phi, \{\mathbf{W}\}^T_{t=1}, \{\mathbf{C}\}^T_{t=1}$}
% \end{algorithm}



%%% For algorithmic
% \algrenewcommand\algorithmicrequire{\textbf{Input:}}
% \algrenewcommand\algorithmicensure{\textbf{Return:}}

% \begin{algorithm}
% \caption{: Training algorithm for \textsc{CascadeXML}}\label{alg:cap}
% \begin{algorithmic}[1]
% \Require{X, Y}
% \State $\hat{\mathbf{Z}}_l = \mathbf{v}_l/\left\lVert \mathbf{v}_l \right\rVert \textrm{; where} \; \mathbf{v}_l = \sum_{i:y_{i,l}=1}\Phi_{tfidf}(\mathbf{x}_i), \; \forall l \in [L]$
% \State $\{\mathbf{C}^t\}_{t=1}^{T} \gets \textrm{2-means-clustering}(\hat{\mathbf{Z})}$
% \State $ \textrm{Generate} \{\mathbf{Y}^t\}_{t=1}^{T}$
% \While{$\textrm{not convergence}$}
%     \State $\mathbf{E} \gets \Phi(\mathbf{X})$
%     \State $\textrm{loss} \gets 0$
%     \For{$t \; \textrm{in} \; 1,2,...T$}
%         \If{$t = 1$}
%             \State $\mathbf{P}^t \gets \mathbf{W}^t \mathbf{E}^t$
%         \Else
%             \State $\mathbf{M}^t \gets \textrm{binarize}(\mathbf{P}^{t-1}\mathbf{C}^{t-1,t}) + \mathbf{Y}^t$
%             \LineComment{Use only shortlisted weights for forward pass}
%             \For{$i \; \textrm{in} \; 1,2,...N$}
%                 \For{$j \; \textrm{in} \; 1,2,...K^t$}
%                     \If{$\mathbf{M}^t_{i,j} \neq 0$}
%                         \State $\mathbf{P}^t_{i,j} \gets \mathbf{W}^t_j \mathbf{E}^t_i$
%                     \Else
%                         \State $\mathbf{P}^t_{i,j} \gets 0$
%                     \EndIf
%                 \EndFor
%             \EndFor
%         \EndIf
%         \State $\textrm{loss} \gets \textrm{loss} + \alpha^t\mathcal{L}(\mathbf{P}^t, \mathbf{Y}^t)$
%         \State $\mathbf{P}^t \gets \textrm{Top}(\mathbf{P}^t, \; k^t)$
%     \EndFor
%     \State $\Phi, \{\mathbf{W}\}^T_{t=1} \gets \textrm{argmin}_{\Phi, \{\mathbf{W}\}^T_{t=1}}\textrm{loss}$
% \EndWhile
% \Ensure{$\Phi, \{\mathbf{W}\}^T_{t=1}, \{\mathbf{C}\}^T_{t=1}$}
% % \Ensure{} % this is OK also
% \end{algorithmic}

% \end{algorithm}

==> Shortlist_func.tex <==
\begin{algorithm}
\SetKwInput{KwData}{Input}
\SetKwInput{KwResult}{Return}
\DontPrintSemicolon
\SetNoFillComment
\caption{Shortlisting Function}\label{alg:shortlist}
\KwData{M: Matrix, S: Shortlist}
$\mathbf{M}_s \gets \textrm{Empty List} $

\For{$i \in \mathbf{S}$}{
    \If{$\mathbf{S}_{i} \neq 0$}{
        $\mathbf{M}_s \gets \mathbf{M}_i$\;
    }
}
\KwResult{$\mathbf{M}_s$ : Matrix with only shortlisted rows}
\end{algorithm}


==> Training.tex <==
\section{Training}
We obtain best results with a 4 layer tree structure. The size of cluster and top-K predictions shortlisted at each level for each dataset is provided in Table-<n>. Each level is trained with binary cross entropy loss. We perform a weighted sum of the loss at each level to get the final loss. The weight of each loss is proportional to the <something>. 

We use a 3-phase learning rate schedule which we find to be quite beneficial for training the transformer model. The schedule warms up from a lower learning rate and linearly increases to a maximum over 3 epochs. We maintain the maximum learning rate for 9 epochs. Finally, we cosine anneal the learning rate to a minimum value over 3 epochs. We also use discriminative learning rates for the layers such that our transformer backbone has 1/10th the learning rate of the classifier layers. 

% 311 structure, no cn hidden, dropouts, weight decay, swa does not help


==> commented.tex <==
% \input{Sections/Training}

% \begin{abstract}
%   The abstract paragraph should be indented \nicefrac{1}{2}~inch (3~picas) on
%   both the left- and right-hand margins. Use 10~point type, with a vertical
%   spacing (leading) of 11~points.  The word \textbf{Abstract} must be centered,
%   bold, and in point size 12. Two line spaces precede the abstract. The abstract
%   must be limited to one paragraph.
% \end{abstract}


% \section{Submission of papers to NeurIPS 2022}


% Please read the instructions below carefully and follow them faithfully.


% \subsection{Style}


% Papers to be submitted to NeurIPS 2022 must be prepared according to the
% instructions presented here. Papers may only be up to {\bf nine} pages long,
% including figures. Additional pages \emph{containing only acknowledgments and
% references} are allowed. Papers that exceed the page limit will not be
% reviewed, or in any other way considered for presentation at the conference.


% The margins in 2022 are the same as those in 2007, which allow for $\sim$$15\%$
% more words in the paper compared to earlier years.


% Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
% NeurIPS website as indicated below. Please make sure you use the current files
% and not previous versions. Tweaking the style files may be grounds for
% rejection.


% \subsection{Retrieval of style files}


% The style files for NeurIPS and other conference information are available on
% the World Wide Web at
% \begin{center}
%   \url{http://www.neurips.cc/}
% \end{center}
% The file \verb+neurips_2022.pdf+ contains these instructions and illustrates the
% various formatting requirements your NeurIPS paper must satisfy.


% The only supported style file for NeurIPS 2022 is \verb+neurips_2022.sty+,
% rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
%   Microsoft Word, and RTF are no longer supported!}


% The \LaTeX{} style file contains three optional arguments: \verb+final+, which
% creates a camera-ready copy, \verb+preprint+, which creates a preprint for
% submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
% \verb+natbib+ package for you in case of package clash.


% \paragraph{Preprint option}
% If you wish to post a preprint of your work online, e.g., on arXiv, using the
% NeurIPS style, please use the \verb+preprint+ option. This will create a
% nonanonymized version of your work with the text ``Preprint. Work in progress.''
% in the footer. This version may be distributed as you see fit. Please \textbf{do
%   not} use the \verb+final+ option, which should \textbf{only} be used for
% papers accepted to NeurIPS.


% At submission time, please omit the \verb+final+ and \verb+preprint+
% options. This will anonymize your submission and add line numbers to aid
% review. Please do \emph{not} refer to these line numbers in your paper as they
% will be removed during generation of camera-ready copies.


% The file \verb+neurips_2022.tex+ may be used as a ``shell'' for writing your
% paper. All you have to do is replace the author, title, abstract, and text of
% the paper with your own.


% The formatting instructions contained in these style files are summarized in
% Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.


% \section{General formatting instructions}
% \label{gen_inst}


% The text must be confined within a rectangle 5.5~inches (33~picas) wide and
% 9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
% type with a vertical spacing (leading) of 11~points.  Times New Roman is the
% preferred typeface throughout, and will be selected for you by default.
% Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
% indentation.


% The paper title should be 17~point, initial caps/lower case, bold, centered
% between two horizontal rules. The top rule should be 4~points thick and the
% bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
% below the title to rules. All pages should start at 1~inch (6~picas) from the
% top of the page.


% For the final version, authors' names are set in boldface, and each name is
% centered above the corresponding address. The lead author's name is to be listed
% first (left-most), and the co-authors' names (if different address) are set to
% follow. If there is only one co-author, list both author and co-author side by
% side.


% Please pay special attention to the instructions in Section \ref{others}
% regarding figures, tables, acknowledgments, and references.


% \section{Headings: first level}
% \label{headings}


% All headings should be lower case (except for first word and proper nouns),
% flush left, and bold.


% First-level headings should be in 12-point type.


% \subsection{Headings: second level}


% Second-level headings should be in 10-point type.


% \subsubsection{Headings: third level}


% Third-level headings should be in 10-point type.


% \paragraph{Paragraphs}


% There is also a \verb+\paragraph+ command available, which sets the heading in
% bold, flush left, and inline with the text, with the heading followed by 1\,em
% of space.


% \section{Citations, figures, tables, references}
% \label{others}


% These instructions apply to everyone.


% \subsection{Citations within the text}


% The \verb+natbib+ package will be loaded for you by default.  Citations may be
% author/year or numeric, as long as you maintain internal consistency.  As to the
% format of the references themselves, any style is acceptable as long as it is
% used consistently.


% The documentation for \verb+natbib+ may be found at
% \begin{center}
%   \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
% \end{center}
% Of note is the command \verb+\citet+, which produces citations appropriate for
% use in inline text.  For example,
% \begin{verbatim}
%   \citet{hasselmo} investigated\dots
% \end{verbatim}
% produces
% \begin{quote}
%   Hasselmo, et al.\ (1995) investigated\dots
% \end{quote}


% If you wish to load the \verb+natbib+ package with options, you may add the
% following before loading the \verb+neurips_2022+ package:
% \begin{verbatim}
%   \PassOptionsToPackage{options}{natbib}
% \end{verbatim}


% If \verb+natbib+ clashes with another package you load, you can add the optional
% argument \verb+nonatbib+ when loading the style file:
% \begin{verbatim}
%   \usepackage[nonatbib]{neurips_2022}
% \end{verbatim}


% As submission is double blind, refer to your own published work in the third
% person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
% previous work [4].'' If you cite your other papers that are not widely available
% (e.g., a journal paper under review), use anonymous author names in the
% citation, e.g., an author of the form ``A.\ Anonymous.''


% \subsection{Footnotes}


% Footnotes should be used sparingly.  If you do require a footnote, indicate
% footnotes with a number\footnote{Sample of the first footnote.} in the
% text. Place the footnotes at the bottom of the page on which they appear.
% Precede the footnote with a horizontal rule of 2~inches (12~picas).


% Note that footnotes are properly typeset \emph{after} punctuation
% marks.\footnote{As in this example.}


% \subsection{Figures}


% \begin{figure}
%   \centering
%   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%   \caption{Sample figure caption.}
% \end{figure}


% All artwork must be neat, clean, and legible. Lines should be dark enough for
% purposes of reproduction. The figure number and caption always appear after the
% figure. Place one line space before the figure caption and one line space after
% the figure. The figure caption should be lower case (except for first word and
% proper nouns); figures are numbered consecutively.


% You may use color figures.  However, it is best for the figure captions and the
% paper body to be legible if the paper is printed in either black/white or in
% color.


% \subsection{Tables}


% All tables must be centered, neat, clean and legible.  The table number and
% title always appear before the table.  See Table~\ref{sample-table}.


% Place one line space before the table title, one line space after the
% table title, and one line space after the table. The table title must
% be lower case (except for first word and proper nouns); tables are
% numbered consecutively.


% Note that publication-quality tables \emph{do not contain vertical rules.} We
% strongly suggest the use of the \verb+booktabs+ package, which allows for
% typesetting high-quality, professional tables:
% \begin{center}
%   \url{https://www.ctan.org/pkg/booktabs}
% \end{center}
% This package was used to typeset Table~\ref{sample-table}.


% \begin{table}
%   \caption{Sample table title}
%   \label{sample-table}
%   \centering
%   \begin{tabular}{lll}
%     \toprule
%     \multicolumn{2}{c}{Part}                   \\
%     \cmidrule(r){1-2}
%     Name     & Description     & Size ($\mu$m) \\
%     \midrule
%     Dendrite & Input terminal  & $\sim$100     \\
%     Axon     & Output terminal & $\sim$10      \\
%     Soma     & Cell body       & up to $10^6$  \\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \section{Final instructions}


% Do not change any aspects of the formatting parameters in the style files.  In
% particular, do not modify the width or length of the rectangle the text should
% fit into, and do not change font sizes (except perhaps in the
% \textbf{References} section; see below). Please note that pages should be
% numbered.


% \section{Preparing PDF files}


% Please prepare submission files with paper size ``US Letter,'' and not, for
% example, ``A4.''


% Fonts were the main cause of problems in the past years. Your PDF file must only
% contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
% achieve this.


% \begin{itemize}


% \item You should directly generate PDF files using \verb+pdflatex+.


% \item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
%   menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
%   also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
%   available out-of-the-box on most Linux machines.


% \item The IEEE has recommendations for generating PDF files whose fonts are also
%   acceptable for NeurIPS. Please see
%   \url{http://www.emfield.org/icuwb2010/downloads/IEEE-PDF-SpecV32.pdf}


% \item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
%   "solid" shapes instead.


% \item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
%   the equivalent AMS Fonts:
% \begin{verbatim}
%   \usepackage{amsfonts}
% \end{verbatim}
% followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
% for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
% workaround for reals, natural and complex:
% \begin{verbatim}
%   \newcommand{\RR}{I\!\!R} %real numbers
%   \newcommand{\Nat}{I\!\!N} %natural numbers
%   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
% \end{verbatim}
% Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.


% \end{itemize}


% If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
% you to fix it.


% \subsection{Margins in \LaTeX{}}


% Most of the margin problems come from figures positioned by hand using
% \verb+\special+ or other commands. We suggest using the command
% \verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
% figure width as a multiple of the line width as in the example below:
% \begin{verbatim}
%   \usepackage[pdftex]{graphicx} ...
%   \includegraphics[width=0.8\linewidth]{myfile.pdf}
% \end{verbatim}
% See Section 4.4 in the graphics bundle documentation
% (\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})


% A number of width problems arise when \LaTeX{} cannot properly hyphenate a
% line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
% necessary.


% \begin{ack}
% Use unnumbered first level headings for the acknowledgments. All acknowledgments
% go at the end of the paper before the list of references. Moreover, you are required to declare
% funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
% More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2022/PaperInformation/FundingDisclosure}.


% Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
% \end{ack}
